View Selection with Geometric Uncertainty Modeling

Estimating positions of world points from features observed in images is a key problem in 3D reconstruction, image mosaicking,simultaneous localization and mapping and structure from motion. We consider a special instance in which there is a dominant ground plane $\mathcal{G}$ viewed from a parallel viewing plane $\mathcal{S}$ above it. Such instances commonly arise, for example, in aerial photography. Consider a world point $g \in \mathcal{G}$ and its worst case reconstruction uncertainty $\varepsilon(g,\mathcal{S})$ obtained by merging \emph{all} possible views of $g$ chosen from $\mathcal{S}$. We first show that one can pick two views $s_p$ and $s_q$ such that the uncertainty $\varepsilon(g,\{s_p,s_q\})$ obtained using only these two views is almost as good as (i.e. within a small constant factor of) $\varepsilon(g,\mathcal{S})$. Next, we extend the result to the entire ground plane $\mathcal{G}$ and show that one can pick a small subset of $\mathcal{S'} \subseteq \mathcal{S}$ (which grows only linearly with the area of $\mathcal{G}$) and still obtain a constant factor approximation, for every point $g \in \mathcal{G}$, to the minimum worst case estimate obtained by merging all views in $\mathcal{S}$. Finally, we present a multi-resolution view selection method which extends our techniques to non-planar scenes. We show that the method can produce rich and accurate dense reconstructions with a small number of views. Our results provide a view selection mechanism with provable performance guarantees which can drastically increase the speed of scene reconstruction algorithms. In addition to theoretical results, we demonstrate their effectiveness in an application where aerial imagery is used for monitoring farms and orchards.

==> camgrid.tex <==
\section{Sensor Selection for the Entire Scene}\label{sec:camgrid}

In the previous section, we established that for a world point $g$, the optimal pair of cameras can produce a reconstruction with approximation ratio less than $\sqrt{\frac{1+2\alpha}{1-4\alpha}}$ (Theorem~\ref{thrm:opt2cameras3dbound}).
However, if we use this directly for every scene point, we may end up choosing two cameras for each scene point, which in turn might result in a large number of cameras.

 \begin{figure}[h]
 \centering
 	\includegraphics[width=0.5\textwidth]{fig/camgrid.png}
 	\caption{The square sensor grid in 3D}
 	\label{fig:grid}
 \end{figure}


In this section, we show that a coarse grid of cameras provide a good reconstruction for every scene point.

Recall that $\mathcal{G}$ is the ground plane, $\mathcal{S}$ is the view plane,   $\mathcal{G}$ is parallel to  $\mathcal{P}$ and the distance between them is $h$. 
Let $\mathcal{\overline{S}}$ be a square grid imposed on $\mathcal{S}$ with resolution $\delta_d$, which is shown in Fig~\ref{fig:grid}. The same grid $\mathcal{\overline{G}}$ is also imposed on the ground plane $\mathcal{G}$. 
To demonstrate the main strategy at a high-level, consider a ground point $g \in \mathcal{G}$, where we can find the optimal pair of cameras in the corse camera grid $\mathcal{\overline{S}}$. By moving the ground point in a region $\mathcal{R}(g)$ and using the same pair of cameras, we establish an upper bound of any points in the region $\mathcal{R}(g)$.

In this section, we make this rough argument concrete. Specifically, we show that 
with the choice of $\delta_d = \frac{h}{\tan(\pi/4-\alpha)}$, we achieve a $2$ approximation ratio for uncertainty everywhere using 
$|\mathcal{\overline{S}}| = \lceil \frac{9Area(\mathcal{G})}{h^2} \rceil$ cameras.
Due to space limitations, we present the lemmas and main ideas and leave detailed proofs to the supplementary material.

\subsection{Problem 2 in 2D}
For cameras in the grid $s \in \overline{S}$ and target $g \in G$, we define the grid uncertainty $\overline{\varepsilon}(g)$ using only the best two cameras in grid $\overline{S}$ as the following
$$
\overline{\varepsilon}(g) = \min_{s_i, s_j \in \overline{S}}\varepsilon(g,\{s_i,s_j\}) 
$$
As mentioned earlier, we will choose the grid resolution to be $\delta_d = \frac{h}{\tan(\pi/4-\alpha)}$ which is half of the distance between the optimal pair of cameras. 


\begin{lemma}\label{lem:gridu}
The minimum worst case uncertainty of any point $g$ is given as $\varepsilon_\infty$,
we claim that $\forall g \in \overline{G}$
$$
\overline{\varepsilon}(g) \leq \sqrt{\frac{1+2\alpha}{1-4\alpha}} \cdot \varepsilon_\infty
$$ 
\end{lemma}

In order to bound the uncertainty of any target $\forall g \in G$ using the camera grid $\overline{S}$, we need to explore the uncertainty of the targets in between the grid. Therefore, we fix a grid point and define a range of targets $R(g) = [g-\delta_d/2, g+\delta_d/2]$ such that $R(g)$ is generated by moving $g \in \overline{G}$ along the $x$-axis of the grid as shown in Fig~\ref{fig:grid3dv2}. We now show that the worst case uncertainty is achieved at the end points of this interval (i.e. the midpoint of two grid locations). We do this in two parts: first, we show that the sum of the viewing angles increases as we move away from a grid point until we reach to the midpoint. Next, we use this result to upper bound the uncertainty. 

\begin{lemma}\label{lem:maxtheta}
Let $g \in \overline{G}$ be a grid location with grid uncertainty $\overline{\varepsilon}(g)$ using the optimal pair of cameras $\{s_i,s_j\}$ with orientation $\theta_i,\theta_j$ respectively.  For any $g' \in R(g) = [g-\delta_d/2, g+\delta_d/2]$, 
$s_i$ and $s_j$ view $g'$ at an angle at most $\theta_i + \theta_j$ is maximized. This value is achieved when the inner half-plane of $Cone_i$ and $Cone_j$ intersects $g \pm \delta_d/2$.
\end{lemma}

It turns out that computing the uncertainty directly, as we did for a single point is tricky because the change in the viewing angles is monotonic.
Instead we show that $\theta_i+\theta_j$ is monotonic and further, there is a function $\xi(g)$ which increase monotonically with $\theta_i+\theta_j$ and upper bounds $\overline{\varepsilon}(g)$ -- i.e .$\overline{\varepsilon}(g) \leq \xi(g)$ for all $g$. This yields our main result:

\begin{theorem}\label{thrm:grid3d1}
For all targets $g \in G$, the worst case grid uncertainty is bounded as follows
$$
\overline{\varepsilon}(g) \leqslant 1.75 \varepsilon_\infty
$$
\end{theorem}

\subsection{Problem 2 in 3D}

In 3D, we use the same grid resolution $\delta_d = \frac{h}{\tan(\pi/4-\alpha)}$ for the this section, which is half of the distance between the optimal pair of cameras. The main result is

\begin{theorem}\label{thrm:grid3d2}
For all targets $g \in \mathcal{G}$, the worst case grid uncertainty is bounded as follows
$$
\overline{\varepsilon}(g) \leqslant 2 \varepsilon_\infty
$$
\end{theorem}

The proof is similar to the 2D case. It is extended to include perturbations in both $x$ and $y$ directions which slightly increases the bounds.
See Figures~\ref{fig:camgridtopdown} and \ref{fig:grid3dv2}.

\begin{figure}[h]
\centering
	\includegraphics[width=0.5\textwidth]{fig/camgridtopdown2.png}
	\caption{Camera grid: top down view}
	\label{fig:camgridtopdown}
\end{figure} 

\begin{figure}[h]
\centering
	\includegraphics[width=0.4\textwidth]{fig/grid3dv2.png}
	\caption{Camera grid in 3D: $g$ is perturbed to $g^*$ to achieve maximum uncertainty.}
	\label{fig:grid3dv2}
\end{figure} 


==> twosensors.tex <==
\section{Two Sensors Bound}
In order to achieve $\varepsilon_\infty$ in 3-D, the number of cameras required is unbounded. 
In this section, we explore the uncertainty $\varepsilon_{pq}$ using only two sensors $s_p$ and $s_q$, which achieves $\varepsilon_{pq} \leq 1.5 \varepsilon_\infty$.

\subsection{Two Dimensions}
We start with the planar case. The cameras and target will appear on the lines $g \in G$ and $s \in S$ respectively and the distance between $G$ and $S$ remains to be $h$ as the height.

We set the coordinate system on target $g = [0,0]$ with $x$-axis being parallel to $G$. Let $s_p = [-h,h]$ and $s_q = [h,h]$ be two cameras and their angles are $\theta_p$,$\theta_q$ respectively. The vertices of the convex polygon $Q'$ are $\{v_1,v_2,v_3,v_4\}$. 

\begin{lemma}\label{lem:angle2d}
$\overline{t_1t_3} > \overline{t_2t_4}$ when $\theta_1 + \theta_2 - 2\alpha \geqslant \pi/2$ as shown in Fig~\ref{fig:acbd}. 
\end{lemma}

\begin{proof}
As shown in Fig~\ref{fig:acbd}, if $\angle eab \geqslant \pi/2$, then we can create $\overline{ab'} \perp \overline{ex}$ and $\overline{cd'} \perp \overline{fx}$. From the isosceles trapzoid $ab'cd'$, it is clear that $\overline{ac} > \overline{bd}$ since $\overline{ac}$ is the diagonal line. We conclude the proof by showing that $\angle eab = \theta_1+\theta_2-2\alpha$. 
\end{proof}
We will be focusing on the cases when $\theta_1 + \theta_2 -2\alpha \geqslant \pi/2$.
In practice, most of the reliable and trackable image features appear within $\pi/2$ of the camera's field of view while assuming that the camera do not rotate intentionally for any specific target point. Thus, the same target point will be successfully tracked when $\theta_{1,2} > \pi/4$, which leads to $\theta_1+ \theta_2-2\alpha \geqslant \pi/2$ the majority sensing configuration.     
Therefore, we define $u_\alpha(x,\{\theta_1, \theta_2, h \}) = min(\overline{ac})$. 

\begin{figure}[h]
\centering
	\includegraphics[width=0.7\columnwidth]{fig/acne.png}
	\caption{uncertainty model in 2D}
	\label{fig:acbd}
\end{figure} 

%Before analyzing the worse case, a closed form solution is omitted here. We define $u_\alpha(x,\{\theta_1,\theta_2,d\}) = u_\alpha(x,\{e,f\})$ as a function of $\alpha$, $\theta_{1,2}$, and $d$, where $d$ is the distance between the sensor $e$ and $f$.
%Using the law of sine by looking at the triangle $eba$, we can find that $\frac{\overline{ab}}{sin(2\alpha)} = \frac{\overline{ef}}{sin{\angle{ebf}}}$. We can also find out that $\angle{ebf} = \pi - 2\alpha-\angle{eab} = \pi - 2\alpha - (\theta_1 + \theta_2 - 2\alpha) = \pi-\theta_1 - \theta_2$. By looking at triangle 
%$abf$, we know that $\frac{\overline{ea}}{sin(\theta_2-\alpha)} = \frac{d}{sin(\pi-\theta_1-\theta_2+2\alpha)}$. By combining both equations, we can get the following:
%\begin{equation}\label{eq:A}
%l_1 = \overline{ab} = d\frac{sin(\theta_2-\alpha)sin(2\alpha)}{sin(\theta_1+\theta_2-2\alpha)sin(\theta_1+\theta_2)}
%\end{equation}
%Using the same method, we have:
%\begin{equation}\label{eq:B}
%l_2 = \overline{bc} = d\frac{sin(\theta_1+\alpha)sin(2\alpha)}{sin(\theta_1+\theta_2)sin(\theta_1+\theta_2+2\alpha)}
%\end{equation}
%Using and the law of cosine, the uncertainty diameter $u_\alpha(x,\{\theta_1,\theta_2,d\})$ can be calculated as 
%\begin{equation}\label{eq:C}
%u_\alpha(x,\{\theta_1,\theta_2,d\}) = \sqrt{l_1^2+l_2^2-2l_1l_2 cos(\theta_1+\theta_2)}
%\end{equation}
%
%Given Eq~\ref{eq:C}, we can analyze $max(u_\alpha(x,\{\theta_1,\theta_2,d\})$ for fixed sensors and target locations and varying $\theta_{1,2}$.




\subsection{Three Dimensions}

\begin{lemma}
$U_\alpha(x,\{v_1,v_2\}) = u_\alpha(x,\{v_1,v_2\})$
\end{lemma}
 We claim the maximum uncertainty diameter by intersecting two cones originated from $e,f$ is the same as the maximum uncertainty diameter by intersecting two wedges originated from $e,f$ in 2D. 
\begin{proof}
As shown in Fig~\ref{fig:u3d2d}, when we take the isosceles trapezoid $ab'cd'$ and create a truncated cone by rotating around the line $\overline{ex}$, the line $\overline{ac}$ remains the maximum line segments within.  This is because both $\overline{ab'}$ and $\overline{cd'}$ are the diameter created by rotation around $\overline{ex}$. We will call the actual polyhedra created by the two cones intersection as $K$. It is clear that $K$ is at least within one of the uncertainty cones. If other wise, $K$ will be truncated so that it is contained within both cones. Therefore, if we create a plane cut for cone $ecd'$ using two planes perpendicular to the line $\overline{ex}$ at $\overline{ab'},\overline{cd'}$, the truncated cone will include $K$. Thus, $U_\alpha(x,\{e,f\})  = \overline{ac}= u_\alpha(x,\{e,f\})$.
\end{proof}

\begin{figure}[h]
\centering
	\includegraphics[width=0.7\columnwidth]{fig/u3d2d.png}
	\caption{Two Cones intersection uncertainty in 3D}
	\label{fig:u3d2d}
\end{figure} 
